Comprehensive Process Drift Detection with Visual Analytics

Recent research has introduced ideas from concept drift into process mining to enable the analysis of changes in business processes over time. This stream of research, however, has not yet addressed the challenges of drift categorization, drilling-down, and quantification. In this paper, we propose a novel technique for managing process drifts, called Visual Drift Detection (VDD), which fulfills these requirements. The technique starts by clustering declarative process constraints discovered from recorded logs of executed business processes based on their similarity and then applies change point detection on the identified clusters to detect drifts. VDD complements these features with detailed visualizations and explanations of drifts. Our evaluation, both on synthetic and real-world logs, demonstrates all the aforementioned capabilities of the technique.

==> addon/macros-DECLARE-drawing.tex <==
% for file in *.tex; do echo ${file%.*} | sed -e 's/^\(.\)/Draw\u\1/' | sed -e 's/\(.*\)/\\NewDocumentCommand{\\1}{ O{\$\\paramx\$} O{\$\\paramy\$} }{%/'; more "$file" | sed -e 's/\$\\paramx\$/#1/' | sed -e 's/\$\\paramy\$/#2/'; echo '%'; echo '}'; echo;  done > ../draw-Declare-macros.tex
\RequirePackage{xparse}

\NewDocumentCommand{\DrawAbsence}{ +O{$\paramx$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center)]\node[DECLARE.task,DECLARE.existcon=$0..m$]{#1};\end{tikzpicture}%
}

\NewDocumentCommand{\DrawAltprec}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.alt.prec] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawAltresp}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.alt.resp] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawAltsucc}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.alt.succ] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawAtmostone}{ O{$\paramx$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center)]\node[DECLARE.task,DECLARE.existcon=$0..1$]{#1};\end{tikzpicture}%
}

\NewDocumentCommand{\DrawChnprec}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.chn.prec] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawChnresp}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.chn.resp] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawChnsucc}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.chn.succ] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawCoex}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.coex] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawEnd}{ O{$\paramx$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center)]\node[DECLARE.task,DECLARE.existcon=End]{#1};\end{tikzpicture}%
}

\NewDocumentCommand{\DrawExistence}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center)]\node[DECLARE.task,DECLARE.existcon=$n..\ast$]{#1};\end{tikzpicture}%
}

\NewDocumentCommand{\DrawInit}{ O{$\paramx$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center)]\node[DECLARE.task,DECLARE.existcon=Init]{#1};\end{tikzpicture}%
}

\NewDocumentCommand{\DrawNotchnsucc}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.chn.succ,DECLARE.neg] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawNotcoex}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.coex,DECLARE.neg] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawNotsucc}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.succ,DECLARE.neg] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawParticipation}{ O{$\paramx$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center)]\node[DECLARE.task,DECLARE.existcon=$1..\ast$]{#1};\end{tikzpicture}%
}

\NewDocumentCommand{\DrawPrec}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.prec] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawResex}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.resex] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawResp}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.resp] node {} (2);
\end{tikzpicture}%
}

\NewDocumentCommand{\DrawSucc}{ O{$\paramx$} O{$\paramy$} }{%
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=3.5*\DTZU]
 \node[DECLARE.task,] (1) {#1};
 \node[DECLARE.task,right=of 1] (2) {#2};
   
 \path (1) edge [DECLARE.succ] node {} (2);
\end{tikzpicture}%
}

==> addon/macros-DECLARE.tex <==
% \def\LTLFOfrag {\ensuremath{ \prescript{\land}{\circledast}{\forall\LTLf}} }
\def\LTLFOfrag {\ensuremath{\mathcal{L}_{\LTLf}^{\forall \wedge \circledast}}}

%\def\NowCns {\ensuremath{ \prescript{\vartimes\hspace{-1.25ex}\scalebox{0.75}{\lglobally}}{}{\Cns}}}
\def\CnsQu {\ensuremath{\Cns^{\text{q}}}}

\def\ActvSym {\ensuremath{\bullet}}
\def\Actv {\ensuremath{\varPhi_{\ActvSym}}}
\def\Trgt {\ensuremath{\varPhi_\Rightarrow}}
\def\Asgn {\ensuremath{\mathscr{A}}}
\def\Intrp {\ensuremath{\mathscr{I}}}
\def\IntrpA {\ensuremath{\Intrp_{\ActvSym}}}
\def\IntrpT {\ensuremath{\Intrp_\Rightarrow}}
\def\PreCns {\ensuremath{\prescript{\forall}{\Intrp}{\CnsTmp}}}
\def\PreCnsPrime {\ensuremath{\prescript{\forall}{\Intrp'}{\CnsTmp}}}

\def\NowCns {\ensuremath{\Cns^{(\ActvSym)}}}

\RequirePackage{xparse}
\NewDocumentCommand{\ActvC}{o}{%
  \ensuremath{\varphi_\bullet%
    \IfValueT{#1}{(#1)}%
  }%
}
\NewDocumentCommand{\CorrC}{o}{%
  \ensuremath{\varphi_\rightleftharpoons%
    \IfValueT{#1}{(#1)}%
  }%
}
\NewDocumentCommand{\TrgtC}{o}{%
  \ensuremath{\varphi_\Rightarrow%
    \IfValueT{#1}{(#1)}%
  }%
}

\NewDocumentCommand{\DeQuery}{m o}{%
\ensuremath{%
	\left\lbrack%
	#1 | \,%
	\IfValueTF{#2}{%
		#2%
	}{%
		(\CnsQu,\SuppMin,\ConfMin)
	}%
	\right\rbrack
}%
}

\def\ActvLang {\ensuremath{\mathscr{L}_\bullet}}
\def\TrgtLang {\ensuremath{\mathscr{L}_\Rightarrow}}

==> addon/macros-for-requirements-list.tex <==
%
% This one allows us to have a custom DESCRIPTION environment, in which numbers are preceded by a one-letter prefix.
% A short description can be added as an additional parameter to the begin-environment command.
% Successive references will have that very one-letter prefix + number with hyper-reference to it.
%
\RequirePackage{enumitem}
%
\def\requiprefix{R}
%
\newcounter{requicount}
\newlist{requidescr}{description}{1}
\setlist[requidescr,1]{%
	before={\setcounter{requicount}{0}%
		\renewcommand*\therequicount{\arabic{requicount}}},
	,font=\bfseries{\requiprefix}\stepcounter{requicount}\therequicount\normalfont.~\bfseries
}
%
% From https://tex.stackexchange.com/questions/1230/reference-name-of-description-list-item-in-latex
\makeatletter
\def\namedlabel#1{\begingroup
	\def\@currentlabel{\requiprefix\therequicount}%
	\phantomsection\label{#1}\endgroup
}
\makeatother
%
% Usage example:
% \begin{requidescr} % CUSTOM from CDC, with love
%   \item[\namedlabel{req:xaxis} Cluster on Y axis] Something more about that here.
% \end{requidescr}
% I especially like \ref{req:xaxis}.

==> addon/memorandum.tex <==
% !TeX root = ../main.tex
%
\section*{For us authors: some tips and tricks}
\label{sec:memo}
%%%
%%% Start of: preliminary commands to be used exclusively in this file.
%%%
\newglossaryentry{test}{name={test},description={A fictionary test}}
\newacronym{testacro}{TA}{Test Acronym}
%%%
%%% End of: preliminary commands to be used exclusively in this file.
%%%
%
% --------------------------------
% About comments
% --------------------------------
%
\hl{For your comments}, please use the
\todo[inline]{\texttt{todo} environment, either in-line or }
or aside.
\todo{aside}
%
You can even add missing figures with the \verb|\missingfigure| command (see \cref{fig:example:missing:figure}).
\begin{figure}[b]
\missingfigure{\texttt{{\textbackslash}missingfigure} command}
\caption{A missing figure}
\label{fig:example:missing:figure}
\end{figure}
%
\\
%
% --------------------------------
% About inline lists
% --------------------------------
%
\hl{For lowercase-roman-enumerated inline lists}, please use
\begin{iiilist}
\item the
\item \texttt{iiilist}
\item environment.
\end{iiilist}
It is a custom command you find in \verb|addons/commands.tex|. It is based on the \verb|\inparaenum| command, from package \textit{paralist}.
%
\\
%
% --------------------------------
% About keywords
% --------------------------------
%
\hl{For specific terms}, which may change in the future, add a \hl{glossary} entry in \texttt{addons/glossary.tex},
and use
\begin{iiilist}
\item the \texttt{gls} command to use them (e.g., \gls{test}),
\item the \texttt{Gls} command for capitalising them (e.g., \Gls{test}),
\item the \texttt{glspl} command for obtaining their plural form (e.g., \glspl{test}), and
\item the \texttt{Glspl} command for for obtaining their plural capitalised form (e.g., \Glspl{test}).
\end{iiilist}
It turns out to be very useful in those situations in which the co-authors do not remember, for example, whether they should indicate the sequences of executed actions as ``traces'' or ``runs''. To solve the issue and avoid that all co-authors write different things, they can decide on a temporary solution (say, ``traces''), make it a glossary entry (say, \verb+\newglossaryentry{actx}{name={trace},description={...}}+), use \verb+\gls{actx}+ (or similar commands -- see above) every time they want to say that thing, and when the opinion on the best term will change (in favour of ``runs''), it will be enough to change the glossary entry definition (\verb+\newglossaryentry{actxeq}{name={run},description={...}}+) and see it varied everywhere it was used in the text. Another use case is: ``AB Testing'' or ``AB testing''? To avoid that the ``T''s of ``testing'' occur as upper-case sometimes, and as lower-case at times, a single glossary entry comes handy!
%
\\
%
\hl{For acronyms}, they are meant be defined within the same file as follows: \texttt{{\textbackslash}newacronym\{testacro\}\{TA\}\{Test Acronym\}}.
They can be referenced by using \texttt{{\textbackslash}Gls} (plus variants for plural forms etc.).
Result is, you get the full version the first time the acronym is used
-- \texttt{{\textbackslash}gls\{testacro\}} is displayed as \Gls{testacro}.
From the second time onwards, the call will return the acronym only, without any description:
\texttt{{\textbackslash}gls\{testacro\}} is displayed as \Gls{testacro}.
To force the representation to have either long or short versions, use
\texttt{{\textbackslash}acrlong\{testacro\}}
(leading to \acrlong{testacro})
or
\texttt{{\textbackslash}acrshort\{testacro\}}
(displaying \acrshort{testacro}).
Acronyms are collected in \texttt{addons/glossary.tex} too.
%
\\
%
\hl{To refer to sections, tables, figures, etc.}, please use the \texttt{cref} command (e.g., \cref{sec:memo}).
\texttt{Cref} capitalises and expands the specifier of the referred document part (e.g., \Cref{fig:example:missing:figure}). It is best to be used at the beginning of phrases, whereas \texttt{cref} uses the abbreviation (e.g., \cref{fig:example:missing:figure}).

\begin{AuthNote}[CDC][Anything to add?]
	We can also add author's notes with the \verb|\begin{AuthNote}...\end{AuthNote}| environment. The optional parameters can be passed to the environment to add (1) your name tag or any in-line title, and (2) a side-note-like title.
\end{AuthNote}

==> tables/table-example-log.tex <==
%!TEX root = ../main.tex
\renewcommand{\arraystretch}{1.6}
% Alternate row colours
\rowcolors{2}{white}{gray!12.5}
%\begin{tabular}{ l p{3cm} >{{\goodexample}~}l >{{\goodexample}~}l >{{\badexample}~}l c c}
\begin{tabular}{ l l l l l l }
	\toprule
	\textbf{Trace} & 
	\textbf{Activity 1} & 
	\textbf{Activity 2} & 
	\textbf{Activity 3} & 
	\textbf{Activity 4} & 
	\textbf{Activity 5} 
	\\
	\midrule
	
	$1$ & Lodging ticket &  Appeal & Appeal & Payment & Close ticket 
	\\
	$2$ & Lodging ticket &  Appeal & Appeal & No Payment & Close ticket 
	\\
	$3$ & Lodging ticket &  Appeal & Appeal & No Payment & Close ticket 
	\\
	$4$ & Lodging ticket  & Appeal & No Payment & Close ticket & Reopen ticket
	\\
	$5$ & Lodging ticket &  Appeal  & Payment & Close ticket &
	\\
	$6$ & Lodging ticket  & Appeal & No Payment & Close ticket &
	\\

	\bottomrule
\end{tabular}


==> tables/table-parameters.tex <==
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l l l l l l}
	\toprule
	%\textbf{Approach}            &                                                                    \multicolumn{5}{c}{\textbf{Requirements}}                                                                    \\
	%\cmidrule{2-6}               & \textbf{R1}         & \textbf{R2}                                                                                             & \textbf{R3}         & \textbf{R4} & \textbf{R5} \\
	\textbf{Section}              & \textbf{Parameters} & \textbf{Description}                                                                                    & \textbf{Default}    &  \\ \midrule
	\ref{sec:declare:shift}       & \WinSize            & How many traces are used to calculate constraints in one step                                                       & Guideline provided  &  \\
	\ref{sec:declare:shift}       & \WinStep            & After each window is computed, how many traces we skip to move to calculating next window's                  & Guideline provided  &  \\
	\ref{sec:cluster-changepoint} & Cluster Algorithm   & We choose what method to use, to cluster traces into separate drifting groups             & Found optimal       &  \\
	                              & - Method            & Technique of how clustering algorithm calculates distance between clusters                   & Found optimal       &  \\
	                              & - Metric            & How the distance is calculated for two time-series                                                        & Found optimal       &  \\
	                              & - Criteria          & Criteria of cluster cut off                                                                             & Guideline 
provided &  \\
	                              & - Criteria Parameter & The cutoff value for \emph{Criteria} parameter                                                                     &                     &  \\
	\ref{sec:cluster-changepoint} & Sort Method Distance  & Distance metric to use for sorting inside of clusters & Found optimal       &  \\
	\ref{sec:cluster-changepoint} & Change Point Method   & The method to automatically detect drifts                                                               & Found optimal       &  \\
	                              & - CostFunction      & Cost function to calculate optimize cost point search                                                   & Found optimal       &  \\
	                              & - SearchMethod      & Change point search method                                                                              & Found optimal       &  \\ \bottomrule
\end{tabular} 
} 


==> tikzlibraryDECLARE.code.tex <==
%
% This is the DECLARE TikZ library by Claudio Di Ciccio is licensed under a Creative Commons Attribution-ShareAlike 4.0 International License.
% This work is licensed under the Creative Commons Attribution-ShareAlike 4.0 International License. To view a copy of this license, visit http://creativecommons.org/licenses/by-sa/4.0/.
%
% Author: Claudio Di Ciccio
% Website: www.diciccio.net
% Date: 2017/02/08
%
\usetikzlibrary{arrows.meta,decorations.markings}
\def\DTZU {2ex}
\tikzset{
 DECLARE.task/.style={
  rounded corners=1ex,
  minimum width=3em,
  minimum height=1ex,
  align=center,
  font=\sffamily,
  inner sep=5,
  draw
 },
 DECLARE.existcon/.style={
  label={[style=draw,yshift=-1\pgflinewidth]above:{\tiny \textit{#1}}}
 },
 DECLARE.neg/.style={
  semithick,
  postaction={decorate,decoration={markings,
   mark=at position .5 with {\arrow[xshift=0.15*\DTZU]{Bar[width=1.5*\DTZU]}},
   mark=at position .5 with {\arrow[xshift=-0.15*\DTZU]{Bar[width=1.5*\DTZU]}}
  }}
 },
 DECLARE.resex/.style={
  semithick,
  {Circle[length=1*\DTZU,width=1*\DTZU]}-,
  shorten <=-0.5*\DTZU
 },
 DECLARE.resp/.style={
  semithick,rounded corners,
  {Circle[length=1*\DTZU,width=1*\DTZU]}-{Triangle[length=1*\DTZU,width=1*\DTZU]},
  shorten <=-0.5*\DTZU
 },
 DECLARE.alt.resp/.style={
  semithick,rounded corners,
  {Circle[length=1*\DTZU,width=1*\DTZU]}-{Triangle[length=1*\DTZU,width=1*\DTZU]},
  shorten <=-0.5*\DTZU,
  double distance=0.25*\DTZU
 },
 DECLARE.chn.resp/.style={
  semithick,rounded corners,
  preaction={draw, shorten <= -0.5*\DTZU, double distance=0.25*\DTZU, {Circle[length=1*\DTZU,width=1*\DTZU]}-{Triangle[length=1*\DTZU,width=1*\DTZU]}},
  {-{Triangle[length=1*\DTZU,width=1*\DTZU]}}
 },
 DECLARE.prec/.style={
  semithick,rounded corners,
  {-{Triangle[length=1*\DTZU,width=1*\DTZU]Circle[length=1*\DTZU,width=1*\DTZU]}},
  shorten >=-0.5*\DTZU
 },
 DECLARE.alt.prec/.style={
  semithick,rounded corners,
  postaction={draw, shorten >= 0.5*\DTZU, double distance=0.25*\DTZU, {-{Triangle[length=1*\DTZU,width=1*\DTZU]}}},
  {-{Circle[length=1*\DTZU,width=1*\DTZU]}},
  shorten >= -0.5*\DTZU
 },
 DECLARE.chn.prec/.style={
  semithick,rounded corners,
  preaction={draw, shorten >= 0.5*\DTZU, double distance=0.25*\DTZU, {-{Triangle[length=1*\DTZU,width=1*\DTZU]}}},
  {-{Circle[length=1*\DTZU,width=1*\DTZU]}},
  shorten >= -0.5*\DTZU
 },
 DECLARE.succ/.style={
  semithick,rounded corners,
  {Circle[length=1*\DTZU,width=1*\DTZU]}-{Triangle[length=1*\DTZU,width=1*\DTZU]Circle[length=1*\DTZU,width=1*\DTZU]},
  shorten <=-0.5*\DTZU,
  shorten >=-0.5*\DTZU
 },
 DECLARE.coex/.style={
  semithick,rounded corners,
  {Circle[length=1*\DTZU,width=1*\DTZU]}-{Circle[length=1*\DTZU,width=1*\DTZU]},
  shorten <=-0.5*\DTZU,
  shorten >=-0.5*\DTZU
 },
 DECLARE.alt.succ/.style={
  semithick,rounded corners,
  postaction={draw, shorten >= 0.5*\DTZU, shorten <= -0.5*\DTZU, double distance=0.25*\DTZU, {Circle[length=1*\DTZU,width=1*\DTZU]}-{Triangle[length=1*\DTZU,width=1*\DTZU]}},
  {-{Circle[length=1*\DTZU,width=1*\DTZU]}},
  shorten >= -0.5*\DTZU
 },
 DECLARE.chn.succ/.style={
  semithick,rounded corners,
  preaction={draw, shorten >= 0.5*\DTZU, shorten <= -0.5*\DTZU, double distance=0.25*\DTZU, {Circle[length=1*\DTZU,width=1*\DTZU]}-{Triangle[length=1*\DTZU,width=1*\DTZU]}},
  {-{Circle[length=1*\DTZU,width=1*\DTZU]}},
  shorten >= -0.5*\DTZU
 }
}
